GPUMC: A Stateless Model Checker for GPU Weak Memory Concurrency

GPU computing is embracing weak memory concurrency for performance improvement. However, compared to CPUs, modern GPUs provide more fine-grained concurrency features such as scopes, have additional properties like divergence, and thereby follow different weak memory consistency models. These features and properties make concurrent programming on GPUs more complex and error-prone. To this end, we present GPUMC, a stateless model checker to check the correctness of GPU shared-memory concurrent programs under scoped-RC11 weak memory concurrency model. GPUMC explores all possible executions in GPU programs to reveal various errors - races, barrier divergence, and assertion violations. In addition, GPUMC also automatically repairs these errors in the appropriate cases. We evaluate GPUMC with benchmarks and real-life GPU programs. GPUMC is efficient both in time and memory in verifying large GPU programs where state-of-the-art tools are timed out. In addition, GPUMC identifies all known errors in these benchmarks compared to the state-of-the-art tools.

==> dpor.tex <==

% \input{seg-dpor-example}

\section{$\projname$ : Model Checking under $\srcmm$}
\label{sec:dpor}
In this section we discuss the $\projname$ approach in \Cref{subsec:dpor} followed by a running example in \Cref{subsec:door:example}. Finally, in \Cref{subsec:door:theorems} we discuss the soundness, completeness, and optimality of the proposed exploration algorithm. 
\subsection{DPOR Algorithm}
\label{subsec:dpor}
%\scomment{We have already mentioned that GPUMC extends Trust in the introduction.}
$\projname$ extends GenMC-TruSt and is in the same spirit as other well known dynamic partial order reduction (DPOR) algorithms \cite{DBLP:conf/popl/FlanaganG05,DBLP:journals/pacmpl/Kokologiannakis18,10.1145/2806886,10.1145/3276505,DBLP:journals/jacm/AbdullaAJS17,DBLP:conf/pldi/Kokologiannakis19,DBLP:journals/pacmpl/Kokologiannakis22}. 
\setlength{\intextsep}{1pt}
\begin{wrapfigure}[31]{r}{0.55\textwidth}
\begin{minipage}{0.55\textwidth}
\input{algo1}
\end{minipage}
\end{wrapfigure}
It verifies a program by exploring all its executions in a systematic manner, ensuring that no execution is visited more than once. Like \cite{DBLP:journals/pacmpl/Kokologiannakis22}, our algorithm also takes only 
polynomial space. 

\underline{Outline} \Cref{alg:alg1} invokes the $\explore$ procedure to explore the executions of input program under $\srcmm$. The $\explore$ procedure uses \Cref{alg:algprfs} to enable a read operation to read-from possible writes and thereby explore multiple executions, \Cref{alg:algisopt} to ensure no execution is explored more than once, and \Cref{alg:algracedetection} to identify and fix errors.   
% \onote{The full algorithm is in Algorithm \ref{alg:alg1}.}  
% \scomment{Provide an outline of the algorithms 1-4 and then explain each algorithm in detail}
% \onote{Main algorithm is Algorithm \ref{alg:alg1}, which invokes $\explore$ procedure to explore the executions of input program under Scoped-RC11.}

\underline{$\explore$ procedure} The $\explore$ procedure explores executions $\G$, starting from an empty execution $\G_{\emptyset}$ where $E = \emptyset$, as long as they are consistent for a given memory model, in this case $\srcmm$ (see \Cref{incons1,incons2,incons3,incons4} of \Cref{alg:alg1}).
%Initially, we invoke $\explore$ with an empty execution $\G_{\emptyset}$ corresponding to $E = \emptyset$.
%The consistency checking procedure is model-dependent, and 
%ours checks the axioms of scoped RC11.
 Next, if some of the threads are  waiting
 at a barrier, while all other threads have finished execution,   
 then we observe a \emph{barrier divergence}, and the execution is said to be 
 $\mathsf{Blocked}$. 
 In a blocked execution, different threads may be waiting at different barriers.
 In this case (line \ref{divergence}), we report the divergence and terminate. Otherwise, we continue exploration by picking the next event (line \ref{nextevent}). This schedules 
 a thread and the next enabled event of that thread.
We use the total order $<_{exe}$ to denote the order in which events are added to the execution.

 The exploration stops if an assertion is violated (line \ref{violate}), or when all events from all threads are explored (line \ref{alldone}). The algorithm reports an error in the first case and in the second case outputs the graph $\G$. 
 

%When all events from all threads are explored (line \ref{alldone}), algorithm outputs explored execution $\G$. 

If the exploration is not complete and the current event $e$ is a write (line \ref{case-write}), then 
the procedure $\checkrace$ detects races due to events conflicting with 
$e$ (line \ref{checkrace}), and also offers to repair them. 
On detecting a race, the algorithm chooses one of the following based on user choice --
%one of the options is enabled before starting the exploration based on user choice   
(i) announce the race and stop exploration, or
(ii) announce the race and continue exploration, or (iii) announce the race and repair the race. 

Apart from calling  $\explore$ recursively (\Cref{exploreafter-co}) after adding the necessary $\co$ edges (line \ref{addCOs}) to $\G$, we check if 
$e$ can be paired with any existing read in $\G$ (line \ref{postponedrfs}). These reads are called ``reversible'' as we can reverse their order in the execution by placing them after the writes they read from. 
On a read event $r$, we consider all possible $\rf$s for $r$  and extend the execution $\G$ to a new execution $\G'$ (\addrf, \cref{addrf}).

\input{algo2}
\input{algo3}

\underline{$\declarepostponed$ procedure}
The procedure pairs all reversible reads $r$ in $\G$ with all same-location write events $w$ (line \ref{reversible-reads}) provided $r$ is not in the  $\po \cup \rf$ prefix of $w$ in $\G$  (line \ref{iterate}), to preserve  
the (No-Thin-Air) axiom. Moreover, a new execution $\G'$ is obtained from $\G$ 
where $r$ reads from $w$ (line \ref{remove-erased}), and all events between $r$ and $w$ which are not $\po \cup \rf$ before $w$ are deleted (line \ref{erased}).

\underline{$\isoptimal$ procedure}
To ensure that no execution is explored twice, the  $\isoptimal$  procedure ensures that all writes in the deleted set are $\co$-maximal  wrt their location, and all reads 
in the deleted set read from $\co$-maximal writes. This is done by lines \ref{eisread} to \ref{line6check}
in  $\isoptimal$.

\underline{$\checkrace$ procedure} We check for races while adding each write $w$ to the execution.  For instance,  assume that all the reads and writes have been explored (\Cref{allwr}). For each event $e'$ in this set which is not related to $w$ by $\hab$, we check if any one of them is non-atomic to expose a \emph{data race}. If both have atomic accesses, we check if they are not scope-inclusive to report a \emph{heterogeneous race} (\Cref{iterate-reads}). Likewise, for each read event added, we consider all explored writes (line \ref{allreads}), and repeat the same check to expose a \emph{data race} or a \emph{heterogeneous race}. 

In addition, we also have an option of repair. In {\tt{Repair}} (line \ref{repair}, $\checkrace$), we either skip and return to $\explore$, or do the following repairs and terminate. 
First, if $e$ and $e'$ respectively have atomic and  non-atomic accesses  with non-inclusive scopes, then we update their scope to make them inclusive : for instance, if $e$,$e'$ are 
in different CTAs, we update their scopes to GPU-level.
Second, if  
at least one of $e, e'$ is a non-atomic access, then we update the 
non-atomic access to relaxed atomic, and update the scopes so that $e$, $e'$ have the same scope to prevent a heterogeneous race between them later. 
However, currently, we do not repair on non-atomic location data types. 
\input{algo4}
%\onote{Our $\checkrace$ algorithm differs from the existing approaches since it involves reporting and repairing heterogeneous races.}

% \onote{\sout{$\projname$ preserves soundness, completeness, and optimality even in the presence of divergence. 
% $\projname$ allows two options: (i) stop the exploration on the detection of divergence or (ii) explore the executions assuming that the thread $t$ blocked at the barrier is terminated. 
% If case (ii) is enabled, $\projname$ ensures that the explored executions are sound, complete (terminates thread $t$ and explores all possible interleavings from other threads) and optimal.}}

\noindent{\bf{Comparison with State-of-the-Art}}. We discuss how our algorithm differs from the existing DPOR algorithms.  The first 
departure comes in the $\explore$ procedure where we perform consistency checking: \Cref{incons1,incons2,incons3,incons4} 
are specific to the Scoped RC11 model which is not handled by any of the existing algorithms including the most recent \cite{DBLP:journals/pacmpl/Kokologiannakis22,abdulla2024parsimonious}, since none of them handle scoped models.   
The $\declarepostponed$ procedure is standard in all DPOR algorithms  and checks if we can pair reads with eligible writes  
which have been explored later. Next we have $\isoptimal$, which ensures that we are optimal while exploring executions: 
here, the optimality check of \cite{abdulla2024parsimonious} is tailored for sequential consistency; we extend 
the optimality checking algorithm for RC11 \cite{DBLP:journals/pacmpl/Kokologiannakis22} to $\srcmm$. While optimality is achieved  
by ensuring $\co$-maximality on writes \cite{DBLP:journals/pacmpl/Kokologiannakis22},  there could be optimal $\co$ orderings that 
are inconsistent in the non-scoped setting, which are consistent in the scoped case which need to be considered to 
achieve completeness. This needed careful handling to achieve polynomial space 
just as \cite{DBLP:journals/pacmpl/Kokologiannakis22}. Finally,  our $\checkrace$ algorithm is novel and 
differs from all existing approaches as it reports and also repairs heterogeneous races.
% \paragraph{An Example}
% We now illustrate how $\projname$ works on an example by considering the program  \ref{prg:dpor}.
% Assume that the assertion violation to check is ${\bf {exists}} (a=1 \wedge b=1)$.  This program has 4 consistent executions under scoped-RC11. 
%We first illustrate how all consistent traces are explored. 
\subsection{Exploring the Executions of \ref{prg:dpor}}
\label{subsec:door:example}
We now illustrate the $\projname$ algorithm on program  \ref{prg:dpor} as a running example. The assertion violation to check is ${\bf {exists}} (a=1 \wedge b=1)$.  
This program has 4 consistent executions under $\srcmm$.

 \noindent  The exploration begins with the empty execution, with no events and all relations being empty.  As we proceed with the exploration, we use numbers $\circledsmall{1},\circledsmall{2},\dots$ to denote the order in which events are added to the execution. 
 Among the enabled events, we have the read from $Y$, namely, $a=Y_\MOna$ in thread $\T_2$ and the write to $X$ in $\T_1$. We add two events for these accesses to the execution (lines \ref{case-read}, \ref{addrf}, \ref{case-write} in $\explore$). 
The read on $Y$ has only the initial value 0 to read from; this is depicted by the $\rf$ edge to $\circledsmall{1}$, obtaining $\G_1$. On each new call to $\explore$, the partial execution is checked for consistency (lines \ref{incons1}-\ref{incons4}). $\G_1$ is consistent. 
\makebox[\textwidth]{
    \begin{minipage}{0.45\textwidth}
        \textcolor{black}{
        \[
        \mytag{SEG}
        \label{prg:dpor}
        \inarrC{
        X=Y=0;
        \\[1.2ex]
        \inparII{
        \T_1\tup{\wg_1, \_}
        \\[1.2ex]
        X^\wg_\MOrel = 1;
        \\[1.1ex]
        Y^\wg_\MOrel = 1;
        }{
        ~~\T_2\tup{\wg_1, \_}
        \\[1.2ex]
        ~~a=Y^\wg_\MOna;
        \\[1.1ex]
        ~~b=X^\wg_\MOacq;
        }
        }
        \]
        }
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\textwidth}
    \centering
    \begin{tikzpicture}[yscale=0.6]
    {
      \node (s) at (2,0.2)  {$[init]$ };
      \node (s11) at (.8,-1)  {$\circledsmall{2}{:}\W^{\wg}_\MOrel(X,1)$};
          \node (ss) at (4,0.2)  {$\G_1$};
      \node (s21) at (3.2,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,0)$};
      \node (s22) at (1.2,-2.5)  {};
    \draw[rf] (s) edge (s21); 
    \node[draw=olive, thick, dotted, fit=(s)(s11)(ss)(s21)(s22),inner sep=0.2pt] {};
    }
    \end{tikzpicture}  
    \end{minipage} 
}
Next, the read event on $X$ from $\T_2$ is added (line \ref{case-read}) having two sources to read from $X$ (line \ref{allw}): the initial write to $X$, and the write event $\circledsmall{2}$. This provides two branches to be explored, with consistent executions 
$\G_2$ and $\G_3$ respectively. 

 \makebox[\textwidth]{
     \begin{tikzpicture}[yscale=0.6]
     {
      \node (g2s) at (0,0)  {$[init]$ };
      \node (g2s11) at (-1,-1)  {$\circledsmall{2}{:}\W^{\wg}_\MOrel(X,1)$};
      \node (g2ss) at (2,0)  {$\G_2$};
            \node (g2s21) at (1.4,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,0)$};
     \node (g2s22) at (1.4,-2.5)  {$\circledsmall{3}{:}\R^{\wg}_\MOacq(X,0)$};
            \draw[rf,bend right=21] (g2s) edge (g2s22);
      \draw[rf] (g2s) edge (g2s21);
      \node (g3s) at (6,0)  {$[init]$ };
      \node (g3s11) at (5,-1)  {$\circledsmall{2}{:}\W^{\wg}_\MOrel(X,1)$};
      \node (g3ss) at (8,0)  {$\G_3$};
            \node (g3s21) at (7.4,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,0)$};
     \node (g3s22) at (7.4,-2.5)  {$\circledsmall{3}{:}\R^{\wg}_\MOacq(X,1)$};
      \draw[rf] (g3s11) edge (g3s22);
      \draw[rf] (g3s) edge (g3s21); 
       \node[draw=olive, thick, dotted, fit=(g2s)(g2s11)(g2ss)(g2s21)(g2s22)(g3s)(g3s11)(g3ss)(g3s21)(g3s22), minimum width=\textwidth ,inner sep=0.2pt] {};
       }
    \end{tikzpicture}   
 \label{fig:ex2:seg}    
}

Next, we add write on $Y$ from $\T_1$ to $\G_2, \G_3$ which results in executions $\G_7$ and $\G_4$ respectively. Both $\G_4$ and $\G_7$ are consistent executions. 
% The write on $Y$ from $\T_1$ is the remaining event to be explored, and 
% adding this to $\G_2, \G_3$ results in executions $\G_7$ and $\G_4$ respectively. Both $\G_4$ and $\G_7$ are consistent executions. 

\makebox[\textwidth]{
     \begin{tikzpicture}[yscale=0.6]
     {
      \node (g7s) at (0,0)  {$[init]$ };
      \node (g7s11) at (-1.2,-1)  {$\circledsmall{2}{:}\W^\wg_\MOrel(X,1)$};
      \node (g7s21) at (1.2,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,0)$};
     \node (g7s22) at (1.2,-2.5)  {$\circledsmall{3}{:}\R^\wg_\MOacq(X,0)$};
  \node (g7s12) at (-1.2,-2.5)  {$\circledsmall{4}{:}\W^\wg_\MOrel(Y,1)$};
      \draw[po] (g7s21) edge (g7s22);
  \draw[po] (g7s11) edge (g7s12);
    \node (g7ss) at (2,0)  {$\G_7$};
         \draw[rf] (g7s) edge (g7s21);
      \draw[rf,bend right=30] (g7s) edge (g7s22);
 %      \node (s4) at (0,-3.2)  {(a)};
% \centering
      \node (g4s) at (6,0)  {$[init]$ };
      \node (g4s11) at (4.8,-1)  {$\circledsmall{2}{:}\W^\wg_\MOrel(X,1)$};
      \node (g4s12) at (4.8,-2.5)  {$\circledsmall{4}{:}\W^\wg_\MOrel(Y,1)$};
      \node (g4s21) at (7.2,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,0)$};
           \node (g4s22) at (7.2,-2.5)  {$\circledsmall{3}{:}\R^\wg_\MOacq(X,1)$};
      \draw[po] (g4s21) edge (g4s22);
      \node (g4ss) at (8,0)  {$\G_4$};
           \draw[po] (g4s11) edge (g4s12);
      \draw[rf] (g4s11) edge (g4s22);
      \draw[rf] (g4s) edge (g4s21); 
      \node[draw=olive, thick, dotted, fit=(g4s)(g4s11)(g4ss)(g4s21)(g4s22)(g4s12)(g7s)(g7s11)(g7ss)(g7s21)(g7s22)(g7s12), minimum width=\textwidth ,inner sep=0.2pt] {};
      }
     % \node(s3) at (-.9, -3.3){$\big\downarrow$};
% \node (s4) at (0,-3.2)  {(b)};
    \end{tikzpicture}   
}
\noindent{\bf{Reversible reads}}.
 In $\G_4$, we observe that the read on $Y$ ($\circledsmall{1}$) can also read from the write $\circledsmall{4}$ which was added 
to the execution later. Enabling $\circledsmall{1}$ to read from $\circledsmall{4}$ involves swapping these two events so that the write 
happens before the corresponding read. 
Since $\circledsmall{2}$ is $\po$-before $\circledsmall{4}$, both of these events must take place 
before the read from $Y$ ($\circledsmall{1}$) for the $\rf$ to be enabled. The read from $X$ ($\circledsmall{3}$) however, 
has no dependence on the events in the first thread and happens after $\circledsmall{1}$. 
Therefore, we can 
delete (line \ref{erased} in $\declarepostponed$)
$\circledsmall{3}$, and add the read from $X$ later, after enabling the $\rf$ from $\circledsmall{4}$ to $\circledsmall{1}$ (line \ref{remove-erased} in $\declarepostponed$). 
The optimality check (line \ref{procisoptimal} in $\declarepostponed$) is passed in this case (see also the paragraph on optimality below) and we obtain execution $\G_5$. 
\setlength{\intextsep}{0.2pt}
\begin{wrapfigure}[6]{r}{0.39\textwidth}
\makebox[0.39\textwidth]{
% \begin{minipage}[t]{0.4\textwidth}
     \begin{tikzpicture}[yscale=0.6]
     {
      \node (s) at (0,0)  {$[init]$ };
      \node (s11) at (-1.2,-1)  {$\circledsmall{2}{:}\W^\wg_\MOrel(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\circledsmall{4}{:}\W^\wg_\MOrel(Y,1)$};
                  \node (s21) at (1.2,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,1 )$};
     \draw[po] (s11) edge (s12);
     \node (ss) at (1.8,0)  {$\G_5$};
    %   \node (s4) at (-0.7,-3.9)  {};
       \draw[rf] (s12) edge (s21); 
       \node[draw=olive, thick, dotted, fit=(s)(s11)(ss)(s21)(s12),inner sep=0.2pt] {};
       }
    \end{tikzpicture}   
% \end{minipage}
}
\end{wrapfigure}
We continue exploring from $\G_5$, adding the read on $X$ (\Cref{case-read} in $\explore$) from $\T_2$.  Here, $X$ may read from (\Cref{allw}, $\explore$) the initial write or $\circledsmall{2}$. This results in executions $\G_6$ and $\G_8$ which are both consistent. 

\makebox[\textwidth]{
 \vspace{0.5em}
     \begin{tikzpicture}[yscale=0.6]
     {
      \node (g8s) at (0,0)  {$[init]$ };
      \node (g8s11) at (-1.2,-1)  {$\circledsmall{2}{:}\W^\wg_\MOrel(X,1)$};
      \node (g8s12) at (-1.2,-2.5)  {$\circledsmall{4}{:}\W^\wg_\MOrel(Y,1)$};
      \node (g8s21) at (1.2,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,1 )$};
     \node (g8s22) at (1.2,-2.5)  {$\circledsmall{5}{:}\R^\wg_\MOacq(X,0)$};
      %\node (s4) at (0,-3.2)  {(d)};
      \draw[po] (g8s21) edge (g8s22);
        \node (g8ss) at (2,0)  {$\G_8$};
     \draw[po] (g8s11) edge (g8s12);
      \draw[rf, bend right=22] (g8s) edge (g8s22);
      \draw[rf] (g8s12) edge (g8s21);
      
      \node (g6s) at (6,0)  {$[init]$ };
      \node (g6s11) at (4.8,-1)  {$\circledsmall{2}{:}\W^\wg_\MOrel(X,1)$};
      \node (g6s12) at (4.8,-2.5)  {$\circledsmall{4}{:}\W^\wg_\MOrel(Y,1)$};
      \node (g6s21) at (7.2,-1)  {$\circledsmall{1}{:}\R^{\wg}_\MOna(Y,1 )$};
     \node (g6s22) at (7.2,-2.5)  {$\circledsmall{5}{:}\R^\wg_\MOacq(X,1)$};
     % \node (s4) at (4,-3.2)  {(c)};
      \draw[po] (g6s21) edge (g6s22);
%      \node (s44) at (-0.7,-3.9)  {};
        \node (g6ss) at (8,0)  {$\G_6$};
     %\draw[po] (s11) edge (s12);
      \draw[rf] (g6s11) edge (g6s22);
      \draw[rf] (g6s12) edge (g6s21); 
      \node[draw=olive, thick, dotted, fit=(g6s)(g6s11)(g6ss)(g6s21)(g6s22)(g6s12)(g8s)(g8s11)(g8ss)(g8s21)(g8s22)(g8s12), minimum width=\textwidth ,inner sep=0.2pt] {};
      }
    \end{tikzpicture}   
}

\noindent{\bf {Optimality}}. From $\G_7$, we do not consider the possibility of $Y$ reading from $\circledsmall{4}$ as it would result in an execution identical to $\G_8$, and consequently violate optimality. 
% as this would affect optimality. 
% Considering this possibility from $\G_7$ will result in an execution identical to $\G_8$ where $X$ reads 0 and $Y$ reads 1 : 
% notice $\G_8$ was obtained by considering this possibility from $\G_4$. 
The $\isoptimal$ procedure checks it to ensure that no execution is explored more than once.  This check enforces a ``$\co$-maximality'' criterion on the events that are deleted while attempting a swap between a read event and a later write event: this is exactly where $\G_4$ and $\G_7$ differ. 
% \scomment{Simplify}
In $\G_7$, while considering the later write on $Y$ ($\circledsmall{4}$) to read from for the read event ($\circledsmall{1}$), the deleted (line \ref{erased}, $\declarepostponed$)
read event on $X$ ($\circledsmall{3}$) reads from the initial write of $X$ which is not $\co$-maximal since it is $\co$-dominated by $\circledsmall{2}$ (lines \ref{eiswrite}-\ref{line6check} in $\isoptimal$). Hence, the check-in line \ref{line6check} of $\isoptimal$ fails. 
In $\G_4$ however, the deleted read on $X$ ($\circledsmall{3}$)  reads from a $\co_x$-maximal write,  and the test passes. 
Thus, the algorithm only considers the possibility 
of the $Y$ reading from $\circledsmall{4}$ in $\G_4$, avoiding redundancy. 




% \noindent{\bf{Reporting errors, races and fixing races}}. The algorithm detects the assertion violation in $\G_6$ (since both $a,b$ read values 1) and terminates.
% Likewise,  the algorithm detects a data race between $\circledsmall{1}$ and $\circledsmall{4}$ in all executions where 
% these are present. We can decide to continue exploration as we have illustrated above after announcing this race, 
% or we can repair it at some point and terminate. Repair will result in changing the non-atomic access of $Y$ in thread 1
% to relaxed atomic access, and make its scope $\wg$. 
% This example 
% does not have barrier divergence. 



\noindent{\bf Program repair}
The exploration algorithm detects the assertion violation in $\G_6$ (since both $a,b$ read values 1) and detects a data race between $\circledsmall{1}$ and $\circledsmall{4}$. 
%The race can be repaired by changing the non-atomic access of $Y$ in thread 1
%to relaxed atomic access. 

% \onote{We allow accesses with non-atomic ordering (inspired by weak access from PTX) on atomic location \cite{Lustig:2019}. 
% Hence, there is a data race between two atomic accesses if at least one of them has non-atomic ordering(to model the data race between weak accesses in PTX and Vulkan).
% We repair this kind of data race by changing the non-atomic ordering to relaxed ordering and making them scope inclusive.
% }

% \sout{Fixing a data race on a non-atomic access on a non-atomic variable automatically faces subtle complexities. Changing the declaration of a non-atomic variable to atomic incurs several non-local changes since all the other non-atomic accesses on this location must be changed. Hence, $\projname$ reports a data race on a non-atomic variable and continues its exploration. }

% It is possible to typecast its access to atomic; however, this may bring new complexities to the compilers. Another approach could be to convert the declaration of the memory location as atomic. However, this repair incurs several non-local changes since the declaration as well as all the other non-atomic accesses on this location must be changed. Hence, $\projname$ reports a data race and continues its exploration. 

If $\projname$ exploration encounters a heterogeneous race between a pair of accesses then $\projname$ automatically repairs the race. To do so, $\projname$ changes the scope of the accesses to enforce an inclusion relation. 
After fixing a heterogeneous race $\projname$ terminates its exploration. 

Consider a variant of the \ref{prg:dpor} program where $T_1$ and $T_2$ are in different CTAs, $\projname$ fixes the heterogeneous race by transforming the scope from $\wg$ to $\gpu$. %If $Y$ is declared as an atomic variable then $\projname$ 
% \sout{If $Y$ had a nonatomic access, then $\projname$ changes it to a relaxed atomic access on $Y$ to fix the data race. 
% The transformed program still has a heterogeneous race on $Y$ since both threads have scope $\cta$, and $\cta_1 \neq \cta_2$.  
% $\projname$ detects this race in the next invocation and repairs the heterogeneous race by upgrading scopes of accesses on $Y$ to $\gpu$.}
% \begin{center}
{
\[
\inarrC{
X=Y=0;
\\[1.2ex]
\inparII{
\T_1\tup{\wg_1, \_}
\\[1.2ex]
X^\wg_\MOrel = 1;
\\[1.1ex]
Y^\wg_\MOrel = 1;
}{
~~\T_2\tup{\wg_2, \_}
\\[1.2ex]
~~a=Y^\wg_\MOna;
\\[1.1ex]
~~b=X^\wg_\MOacq;
}
}
\ \leadsto \
\inarrC{
X=Y=0;
\\[1.2ex]
\inparII{
\T_1\tup{\wg_1, \_}
\\[1.2ex]
{\color{teal}X^\gpu_\MOrel = 1;}
\\[1.1ex]
Y^\wg_\MOrel = 1;
}{
~~\T_2\tup{\wg_2, \_}
\\[1.2ex]
~~a=Y^\wg_\MOna;
% ~~{\color{blue}a=Y^\wg_\MOrlx};
\\[1.1ex]
~~{\color{teal}b=X^\gpu_\MOacq;}
}
}
% \ \leadsto \
% \textcolor{red}{\inarrC{
% X=Y=0;
% \\[1.2ex]
% \inparII{
% \T_1\tup{\wg_1, \_}
% \\[1.2ex]
% X^\gpu_\MOrel = 1;
% \\[1.1ex]
% Y^\gpu_\MOrel = 1;
% }{
% ~~\T_2\tup{\wg_2, \_}
% \\[1.2ex]
% ~~{\color{teal}a=Y^\gpu_\MOrlx};
% \\[1.1ex]
% ~~b=X^\gpu_\MOacq;
% }
% }}
\]
}
% \end{center}
% \[
% \inarrC{
% X=Y=0;
% \\[1.2ex]
% \inparII{
% \T_1\tup{\wg_1, \gpu_1}
% \\[1.2ex]
% X^\wg_\MOrel = 1;
% \\[1.1ex]
% Y^\wg_\MOrel = 1;
% }{
% ~~\T_2\tup{\wg_2, \gpu_1}
% \\[1.2ex]
% ~~a=Y^\wg_\MOna;
% \\[1.1ex]
% ~~b=X^\wg_\MOacq;
% }
% }
% \ \leadsto \
% \inarrC{
% X=Y=0;
% \\[1.2ex]
% \inparII{
% \T_1\tup{\wg_1, \gpu_1}
% \\[1.2ex]
% X^\gpu_\MOrel = 1;
% \\[1.1ex]
% Y^\wg_\MOrel = 1;
% }{
% ~~\T_2\tup{\wg_2, \gpu_1}
% \\[1.2ex]
% ~~a=Y^\wg_\MOrlx;
% \\[1.1ex]
% ~~b=X^\gpu_\MOacq;
% }
% }
% \]










 


\subsection{Soundness, Completeness and Optimality}
\label{subsec:door:theorems}
\begin{theorem}
    The DPOR algorithm for $\srcmm$ is sound, complete and optimal. 
\end{theorem}

%\onote{$\projname$ inherits its optimality from \cite{DBLP:journals/pacmpl/Kokologiannakis22}. }

\noindent{\bf{Soundness}}. The algorithm does not continue exploration from any inconsistent execution as ensured by \Cref{incons1,incons2,incons3,incons4} in \Cref{alg:alg1}, and is therefore sound.

\noindent{\bf{Completeness}}. The DPOR algorithm is complete as it does not miss any consistent and full execution. 
%A full execution is obtained when all threads have executed to completion. 
We prove this in the following steps:
\begin{myitem}
    \item We first show that starting from any consistent execution  $\egraph$,    we can uniquely
    roll back to obtain the  previous execution $\egraph_p$ (see the supplement for the algorithm to compute $\egraph_p$ from $\egraph$). 
    This is proved using  
    the fact that we have a fixed order in exploring the threads, along with the conditions that allow a swap between a read and a later write  
    to take place. To allow a swap of a read $r$ on some variable (say $x$), all events in $\deletedevents$
    respect ``$\co_x$-maximality''. This is enforced by $\isoptimal$  and allows us to uniquely construct the previous execution  $\egraph_p$.
    \item Second, we show that $\explore(\pgm,\egraph_p)$ leads to the call of $\explore(\pgm,\egraph)$.
    This shows that if $\egraph_p$ is reachable by the DPOR algorithm, then $\egraph$ is also reachable.
    % (see Supplement \ref{app:pred}, Lemma \ref{lem:reachblity}).
    \item In the final  step, we show that walking backward from any consistent $\egraph$ 
     we have a unique sequence  of executions $\egraph_p, \egraph_{p-1}, \egraph_{p-2}, \dots, $ 
    till  we obtain the empty execution $\egraph_{\emptyset}$. Thus, starting from $\explore(\pgm,\egraph_\emptyset)$, we obtain $\egraph$.
    % (Supplementary \ref{app:pred},  Lemma \ref{lem:finiteprev}, Lemma \ref{lem:prevseq}).
    
\end{myitem}
\noindent{\bf{Optimality}}. The algorithm is optimal as each full, consistent execution $\egraph$ is generated only once. Lines \ref{exploreafter-rf} and \ref{addCOs} of the $\explore$ procedure ensure that each recursive call to $\explore$ generates an execution that has a different $\rf$ edge or a different $\co$ edge. 
Also, during the $\declarepostponed$ procedure, 
the swap of a read  $r$ with a write  $w$ is successful only when 
the deleted events respect ``$\co_x$-maximality''.
As argued in completeness, for every (partial) consistent execution  $\egraph$, there exists a unique previous consistent execution $\egraph_p$. 

If the algorithm explores $\egraph$ twice, it means that there are two different exploration sequences with respective previous executions  $\egraph_{p}$ and $\egraph_{q}$.
This is a contradiction as we have a unique previous execution.
% (see Supplementary \Cref{app:optmal}, \Cref{thm:optml}).  

\noindent{\bf Polynomial Space}
The DPOR algorithm explores executions recursively in a depth-first manner, with each branch explored independently. 
Since the recursion depth is bounded by the size of the program, this approach ensures that the algorithm uses only polynomial space.

The proofs and related details are provided in the supplementary material \cite{Chakraborty2025}.

\subsection{Exploring the Reads-From Equivalence}
For simplicity, we have focused our presentation on exploring executions that contain the $\co$ relation explicitly.
However, \cref{alg:alg1} can be easily adapted to explore executions where $\co$ is not given explicitly.
This corresponds to exploring the reads-from partitioning~\cite{Chalupa2017}, a setting that is also supported by GenMC~\cite{DBLP:journals/pacmpl/Kokologiannakis22}.
This is often a desirable approach, because it may significantly reduce the search space:~there can be exponentially many executions, differing only in their $\co$, all of which collapse to a single class of the reads-from partitioning.

Exploring the reads-from partitioning requires that every time a new execution is explored, the algorithm performs a consistency check to derive a $\co$, so as to guarantee that the execution is consistent.
If the program has no SC accesses, this check is known to be efficient for RC11~\cite{10.1145/3276505,Lahav:2015}, taking essentially linear time~\cite{tunc_optimal_2023}.
These results easily extend to scoped RC11, by adapting the computation of the happens-before relation so as to take the scope inclusion $\incl$ into consideration.
On the other hand, the presence of SC accesses makes the problem intractable~\cite{Gibbons:1997,Mathur:lics2020}, though it remains in polynomial time with a bounded number of threads~\cite{Gibbons:1997,Abdulla:2019b}.



%If we work with $\po$-$\rf$-$\co$ equivalence, then consistency checking is polynomial time, since 
%it boils down to checking the acyclicity of the execution graph. If we go with $\po$-$\rf$ equivalence, 
%and if the program has no SC accesses, then synthesizing $\co$ edges to obtain a consistent execution takes %time polynomial in the number 
%of events of the execution graph. With SC accesses, this is NP-complete. These results for scoped RC11 %consistency checking 
%follow on similar lines from known results for consistency checking of release acquire  %\cite{10.1145/3276505} and sequential consistency \cite{DBLP:journals/pacmpl/AbdullaAJLNS19}. 
%The main difference 
%with scoped RC11 is in computing the happens-before relation which takes the scope inclusion $\incl$ into consideration. 
















            

==> fig-axioms.tex <==
\begin{center}
\begin{minipage}{0.2\linewidth}   
\flushleft
\begin{tikzpicture}[yscale=0.9]
%     \begin{tikzpicture}[yscale=0.9]
      \node (a) at (0,0)  {$a$};
      \node (b) at (0,-1.5)  {$b$};
      \draw[hb,bend right=30] (a) edge node[left]{$\lhb$} (b);
      \draw[eco,bend right=30] (b) edge node[right,pos=0.2]{$\eco^?$} (a);
 \end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.24\linewidth}    
\flushright
\begin{tikzpicture}[yscale=0.9]
%     \begin{tikzpicture}[yscale=0.9]
      \node (a) at (0,0)  {$r$};
      \node (b) at (0,-1.5)  {$w$};
      \node (c) at (1,-0.7)  {$w'$};
      \draw[rmw] (a) edge node[left,pos=0.2]{$\rmw$} (b);
      \draw[fr] (a) edge node[above]{$\fr$} (c);
      \draw[fr] (c) edge node[below]{$\co$} (b);
 \end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.22\linewidth}   
\flushright
\begin{tikzpicture}[yscale=0.9]
      \node (a) at (0,0)  {$a$};
%      \node (b) at (1,0)  {};
%      \draw[psc,bend right=30] (a) edge node[left]{$\lhb$} (b);
%      \draw[psc,bend right=30] (b) edge node[right]{$\eco$} (a);
%    \draw [--,bend right=80] (a.south) edge (b.south);
%    \draw [po,bend right=80] (b.south) edge (a.south);
    \draw[->,colorPSC,shorten <=5pt,shorten >=5pt](a.center)arc(-180:180:0.5);
    \node at (0.5,-1)  {$\incl \cap \psc$};
 \end{tikzpicture}
\end{minipage}
\hfill
\begin{minipage}{0.3\linewidth}    
\flushright
\begin{tikzpicture}[yscale=0.9]
%     \begin{tikzpicture}[yscale=0.9]
      \node (a) at (0,0)  {$r$};
      \node (b) at (0,-1.5)  {$w$};
      \node (c) at (1.5,0)  {$r'$};
      \node (d) at (1.5,-1.5)  {$w'$};
      \draw[po] (a) edge node[left]{$\po$} (b);
      \draw[rf] (b) edge node[below]{$\rf$} (c);
      \draw[po] (c) edge node[right]{$\po$} (d);
      \draw[rf] (d) edge  (a);
 \end{tikzpicture}
\end{minipage}
\end{center}

==> fig-ex-mp.tex <==
% \begin{figure*}[t]
%     \centering
% \begin{minipage}{0.22\textwidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$[X=Y=0]$ };
%       \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
%       \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
% %
%       \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,0)$};
%       \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,0)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge node[left]{$\po$} (s12);
%       \draw[po] (s21) edge (s22);
%       \draw[rf,bend right=10] (s) edge (s21);
%        \draw[rf,bend right=20] (s) edge node[left]{$\rf$} (s22);
%     \end{tikzpicture}   
% %     \caption{}
% % \label{fig:ex1:mp}    
% \end{minipage}
% \hfill\vline\hfill
% \begin{minipage}{0.22\textwidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$[X=Y=0]$ };
%       \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
%       \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
% %
%       \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,0)$};
%       \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,1)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge (s12);
%       \draw[po] (s21) edge (s22);
%       \draw[rf,bend right=10] (s) edge (s21);
%        \draw[rf,bend right=0] (s11) edge node[left]{$\rf$} (s22);
%     \end{tikzpicture}  
% %     \caption{}
% % \label{fig:ex2:mp}      
% \end{minipage}
% \hfill\vline\hfill
% \begin{minipage}{0.22\linewidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$[X=Y=0]$ };
%       \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
%       \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
% %
%       \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,1)$};
%       \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,1)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge (s12);
%       \draw[po] (s21) edge (s22);
%       \draw[rf] (s12) edge (s21);
%        \draw[rf,bend right=0] (s11) edge (s22);
%     \end{tikzpicture}  
% %     \caption{}
% % \label{fig:ex3:mp}       
% \end{minipage}
% \hfill\vline\hfill 
% \begin{minipage}{0.27\textwidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$i:[X=Y=0]$ };
%       \node (s11) at (-1.2,-1)  {$e_1\!:\!\W^\wg_\MOrlx(X,1)$};
%       \node (s12) at (-1.2,-2.5)  {$e_2\!:\!\W^\wg_\MOrel(Y,0)$};
% %
%       \node (s21) at (1.2,-1)  {$e_3\!:\!\R^\wg_\MOacq(Y,1)$};
%       \node (s22) at (1.2,-2.5)  {$e_4\!:\!\R^\wg_\MOrlx(X,0)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge (s12);
%       \draw[po] (s21) edge (s22);
%       \draw[rf] (s12) edge (s21);
%       \draw[rf,bend right=25] (s) edge (s22);
%       \draw[fr] (s22) edge node[below,pos=0.3]{$\fr$} (s11);
%       \draw[co,bend right=25] (s.west) edge node[left]{$\co$} (s11);
%     \end{tikzpicture}   
%  %     \caption{}
%  % \label{fig:ex4:mp}       
% \end{minipage}
% \caption{Executions for \ref{prg:mp} programs.}
% \label{fig:executions_mp}
% \end{figure*}

\begin{figure}[t]
    \centering
\begin{subfigure}{0.22\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.9]
      \node (s) at (0,0)  {$[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,0)$};
      \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,0)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge node[left]{$\po$} (s12);
      \draw[po] (s21) edge (s22);
      \draw[rf,bend right=10] (s) edge (s21);
       \draw[rf,bend right=20] (s) edge node[left]{$\rf$} (s22);
    \end{tikzpicture}   
     \caption{}
 \label{fig:ex1:mp}    
\end{subfigure}
\hfill\vline\hfill
\begin{subfigure}{0.22\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.9]
      \node (s) at (0,0)  {$[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,0)$};
      \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,1)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[rf,bend right=10] (s) edge (s21);
       \draw[rf,bend right=0] (s11) edge node[left]{$\rf$} (s22);
    \end{tikzpicture}  
     \caption{}
 \label{fig:ex2:mp}      
\end{subfigure}
\\[3ex]
\begin{subfigure}{0.22\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.9]
      \node (s) at (0,0)  {$[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,1)$};
      \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,1)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[rf] (s12) edge (s21);
       \draw[rf,bend right=0] (s11) edge (s22);
    \end{tikzpicture}  
     \caption{}
 \label{fig:ex3:mp}       
\end{subfigure}
\hfill\vline\hfill 
\begin{subfigure}{0.22\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.9]
      \node (s) at (0,0)  {$[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,1)$};
      \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,1)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[sw] (s12) edge (s21);
       \draw[rf,bend right=0] (s11) edge (s22);
    \end{tikzpicture}  
     \caption{}
 \label{fig:ex3:mp}       
\end{subfigure}
\\[3ex]
\begin{subfigure}{0.22\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.9]
      \node (s) at (0,0)  {$i:[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,0)$};
%
      \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,1)$};
      \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,0)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[rf] (s12) edge (s21);
      \draw[rf,bend right=25] (s) edge (s22);
      \draw[fr] (s22) edge node[below,pos=0.3]{$\fr$} (s11);
      \draw[co,bend right=25] (s.west) edge node[left]{$\co$} (s11);
    \end{tikzpicture}   
      \caption{}
  \label{fig:ex4:mp}       
\end{subfigure}
\hfill\vline\hfill 
\begin{subfigure}{0.22\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.9]
      \node (s) at (0,0)  {$i:[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W^\wg_\MOrlx(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W^\wg_\MOrel(Y,0)$};
%
      \node (s21) at (1.2,-1)  {$\R^\wg_\MOacq(Y,1)$};
      \node (s22) at (1.2,-2.5)  {$\R^\wg_\MOrlx(X,0)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[sw] (s12) edge (s21);
      \draw[rf,bend right=25] (s) edge (s22);
      \draw[fr] (s22) edge node[below,pos=0.3]{$\fr$} (s11);
      \draw[co,bend right=25] (s.west) edge node[left]{$\co$} (s11);
    \end{tikzpicture}   
      \caption{}
  \label{fig:ex4:mp}       
\end{subfigure}
\caption{Executions for \ref{prg:smp} programs.}
\label{fig:executions_mp}
\end{figure}



==> fig-mp-rcmm.tex <==
% \begin{figure*}[t]
% \centering
% \begin{subfigure}{0.27\textwidth}
%  \centering
% \[
% \mytag{MP}
% \label{prg:mp}
% \inarrC{
% X=Y=0;
% \\[1.1ex]
% \inparII{
% X_\MOna = 1;
% \\
% Y_\MOrel = 1;
% }{
% a=Y_\MOacq;
% \\
% \Cif(a==1) 
% \\ \quad b=X_\MOna;
% }
% }
% \] 
% \caption{}
% \label{fig:prg:mp}    
% \end{subfigure}
% \hfill\vline\hfill
% \begin{subfigure}{0.2\textwidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$[X=Y=0]$ };
%       \node (s11) at (-1.1,-1)  {$\W_\MOna(X,1)$};
%       \node (s12) at (-1.1,-2.5)  {$\W_\MOrel(Y,1)$};
% %
%       \node (s21) at (1.1,-1)  {$\R_\MOrlx(Y,0)$};
% %      \node (s22) at (1.2,-2.5)  {$\R_\MOrlx(X,1)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge (s12);
% %      \draw[po] (s21) edge (s22);
%       \draw[rf,bend right=10] (s) edge (s21);
% %       \draw[rf,bend right=0] (s11) edge (s22);
%     \end{tikzpicture}  
%     \caption{}
% \label{fig:ex1:mp}      
% \end{subfigure}
% \hfill\vline\hfill
% \begin{subfigure}{0.22\textwidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$[X=Y=0]$ };
%       \node (s11) at (-1.2,-1)  {$\W_\MOna(X,1)$};
%       \node (s12) at (-1.2,-2.5)  {$\W_\MOrel(Y,1)$};
% %
%       \node (s21) at (1.2,-1)  {$\R_\MOacq(Y,1)$};
%       \node (s22) at (1.2,-2.5)  {$\R_\MOna(X,1)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge (s12);
%       \draw[po] (s21) edge (s22);
%       \draw[sw] (s12) edge (s21);
%        \draw[rf] (s11) edgenode[right]{$\rf$} (s22);
%     \end{tikzpicture}  
%     \caption{}
% \label{fig:ex2:mp}       
% \end{subfigure}
% \hfill\vline\hfill 
% \begin{subfigure}{0.27\textwidth}
%  \centering
%      \begin{tikzpicture}[yscale=0.9]
%       \node (s) at (0,0)  {$i:[X=Y=0]$ };
%       \node (s11) at (-1.2,-1)  {$e_1\!:\!\W_\MOna(X,1)$};
%       \node (s12) at (-1.2,-2.5)  {$e_2\!:\!\W_\MOrel(Y,1)$};
% %
%       \node (s21) at (1.2,-1)  {$e_3\!:\!\R_\MOacq(Y,1)$};
%       \node (s22) at (1.2,-2.5)  {$e_4\!:\!\R_\MOna(X,0)$};

%       \draw[po] (s) edge (s11.north) edge (s21.north);
%       \draw[po] (s11) edge (s12);
%       \draw[po] (s21) edge (s22);
%       \draw[sw] (s12) edge (s21);
%       \draw[rf,bend right=25] (s) edge node[right]{$\rf$} (s22);
%       \draw[fr] (s22) edge node[below,pos=0.3]{$\fr$} (s11);
%       \draw[co,bend right=25] (s.west) to node[left]{$\co$} (s11);
%     \end{tikzpicture}   
%     \caption{}
% \label{fig:ex3:mp}       
% \end{subfigure}
% \caption{\ref{prg:mp} program and its executions. RC11 allows the executions in \Cref{fig:ex1:mp,fig:ex2:mp} and forbids the execution in \Cref{fig:ex3:mp}.}
% \label{fig:mp:rcmm}
% \end{figure*}

\begin{figure*}[t]
\centering
\begin{subfigure}{0.2\textwidth}
 \centering
{
\[
% \mytag{MP}
\label{prg:mp}
\inarrC{
X=Y=0;
\\[1.1ex]
\inparII{
X_\MOna = 1;
\\
Y_\MOrel = 1;
}{
a=Y_\MOacq;
\\
\Cif(a==1) 
\\ \quad b=X_\MOna;
}
}
\] 
}
\caption{MP}
\label{fig:prg:mp}    
\end{subfigure}
\hfill
\begin{subfigure}{0.19\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.7,xscale=0.65]
     {
      \node (s) at (0,0)  {$[X=Y=0]$ };
      \node (s11) at (-1.1,-1)  {$\W_\MOna(X,1)$};
      \node (s12) at (-1.1,-2.5)  {$\W_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$\R_\MOacq(Y,0)$};
%      \node (s22) at (1.2,-2.5)  {$\R_\MOrlx(X,1)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
%      \draw[po] (s21) edge (s22);
      \draw[rf,bend right=10] (s) edgenode[left]{$\rf$} (s21); }
%       \draw[rf,bend right=0] (s11) edge (s22);
    \end{tikzpicture}  
    \caption{}
\label{fig:ex1:mp}      
\end{subfigure}
\hfill
\begin{subfigure}{0.2\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.7,xscale=0.65]
     {
      \node (s) at (0,0)  {$[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$\W_\MOna(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$\W_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$\R_\MOacq(Y,1)$};
      \node (s22) at (1.2,-2.5)  {$\R_\MOna(X,1)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[sw] (s12) edge (s21);
       \draw[rf] (s11) edgenode[right]{$\rf$} (s22); }
    \end{tikzpicture}  
    \caption{}
\label{fig:ex2:mp}       
\end{subfigure}
\hfill 
\begin{subfigure}{0.23\textwidth}
 \centering
     \begin{tikzpicture}[yscale=0.7,xscale=0.82]
     {
      \node (s) at (0,0)  {$i:[X=Y=0]$ };
      \node (s11) at (-1.2,-1)  {$e_1\!:\!\W_\MOna(X,1)$};
      \node (s12) at (-1.2,-2.5)  {$e_2\!:\!\W_\MOrel(Y,1)$};
%
      \node (s21) at (1.2,-1)  {$e_3\!:\!\R_\MOacq(Y,1)$};
      \node (s22) at (1.2,-2.5)  {$e_4\!:\!\R_\MOna(X,0)$};

      \draw[po] (s) edge (s11.north) edge (s21.north);
      \draw[po] (s11) edge (s12);
      \draw[po] (s21) edge (s22);
      \draw[sw] (s12) edge (s21);
      \draw[rf,bend right=25] (s) edge node[right]{$\rf$} (s22);
      \draw[fr] (s22) edge node[below,pos=0.3]{$\fr$} (s11);
      \draw[co,bend right=25] (s.west) to node[left]{$\co$} (s11); }
    \end{tikzpicture}   
    \caption{}
\label{fig:ex3:mp}       
\end{subfigure}
\caption{MP program and its executions. RC11 allows the executions in \Cref{fig:ex1:mp,fig:ex2:mp} and forbids the execution in \Cref{fig:ex3:mp}.}
\label{fig:mp:rcmm}
\end{figure*}



==> intro_backup.tex <==
\section{Introduction}
\label{sec:introduction}
In recent years GPUs have emerged as mainstream processing units, more than just an accelerator. Consequently, beyond parallel programming, GPU is becoming an attractive target for shared memory concurrency for further performance gains. 

Writing correct and optimal shared-memory concurrent programs is already a challenging problem for CPUs. In addition to the existing challenges, shared-memory concurrency in GPUs poses new challenges due to different threading paradigms and scoped memory accesses. Unlike CPU threads, the threads in a GPU are organized hierarchically and synchronize in barriers during execution. Moreover, shared-memory accesses are scoped resulting in more fine-grained rules for synchronization, based on the proximity of their threads. 
Although these primitives and rules play a key role in achieving better performance, they are also complex and prone to errors. 

Most of the challenges in ensuring correctness stem from the large number of possible executions of a program and different types of bugs. GPU concurrency may result in various types of concurrency bugs -- assertion violation, data race, heterogeneous race, and barrier divergence. Assertion violation and data race errors are well-known in CPU concurrency as well, however, manifest in more complicated manner in the context of GPU programs. The other two types errors -- heterogeneous race and barrier divergence errors are exhibited in GPU concurrency, unlike CPUs. To catch these errors, it is imperative to explore all possible executions of a program. 
The set of possible executions of a GPU concurrent program is determined by its underlying  consistency model. Under weak consistency, a program may exhibit additional behaviors over interleaving executions, formally known as sequential consistency \cite{lamport-sc}. 
Compared to CPUs, GPU concurrency follows weaker consistency models due to the scoped accesses and their  weaker synchronization rules. 
%As a result, they  allow many more  executions. 
The state-of-the-art approaches do not suffice in identifying these errors under GPU weak memory concurrency. As a result, automated reasoning of GPU concurrency, particularly under weak consistency models, even though a timely and important problem, yet has remained little explored.
To address this gap, in this paper, we develop $\projname$, a model checker for the verification of GPU programs written in scoped C/C++. 


Model checking \cite{DBLP:conf/popl/ClarkeES83} is a technique 
which explores the state space of a program in a systematic manner covering all possible executions of the program. The problem with this approach is that the number 
of executions can grow  exponentially large in the number of concurrent processes. 
Partial order reduction (POR) \cite{DBLP:journals/sttt/ClarkeGMP99,DBLP:books/sp/Godefroid96,DBLP:conf/cav/Peled93}
is an approach which limits the number of explored executions without compromising on system coverage. In POR, the notion of ``equivalent'' 
executions is used, where two executions are equivalent if one can be obtained from the other by swapping independent execution steps which 
come one after the other. 
%Thus, POR enables the partitioning of the entire state space into equivalence classes of executions, 
%and at least one execution per equivalence class is explored. 
Dynamic partial order reduction (DPOR) \cite{DBLP:conf/popl/FlanaganG05} is a technique which explores the execution state space by tracking the equivalence classes on the fly. DPOR is usually coupled with  
Stateless model checking (SMC) \cite{10.1145/263699.263717} to do the exploration without storing the visited states (hence the name ``stateless'').
There are several works on DPOR algorithms for shared memory programs under weak memory 
\cite{DBLP:journals/pacmpl/Kokologiannakis18},\cite{10.1145/2806886}, \cite{10.1145/3276505},\cite{DBLP:journals/jacm/AbdullaAJS17}. 
%DPOR algorithms have also been developed for  weak consistency models such as CC, CCv and CM \cite{DBLP:conf/tacas/AbdullaAKGT23}. 
%These DPOR algorithms are all sound, complete and optimal, although 
%they incur an exponential memory. 
Recently, \cite{DBLP:conf/pldi/Kokologiannakis19}, \cite{DBLP:journals/pacmpl/Kokologiannakis22} proposed a DPOR algorithm which is applicable to a range of weak memory models incurring only polynomial space while being also sound, complete and optimal. All these papers work on  shared memory programs 
and do not address the verification of GPU programs. 

In this paper, we propose a  generic swapping based SMC algorithm to handle GPU programs. 
Each read event in a thread produces many exploration branches, corresponding to each matching write which has been executed in the past. In addition, write events $W$ which are executed after a read event $R$ on a variable $x$ are also considered as potential sources for $R$ to  read from,  by swapping 
$R$ and $W$,  and removing those events which need not happen before $W$. 
Swapping these racy read and write events are done in such a way that the new execution is feasible wrt the underlying memory model, in our case, Scoped RC11, thereby ensuring soundness of our approach. In addition, we also ensure that  the events to be removed 
form a maximal extension of the remaining execution.  
We show  that  maximal extensions always exist and are unique, enabling 
us to prove the completeness and optimality of our approach :  that is, no feasible execution is generated more than once, and no feasible execution is left out.  
Our algorithm has a linear space complexity :   we explore executions in a recursive depth-first manner, where  the recursive depth is bounded by the size of the program. A recursive call requires constant space to represent its difference from the current execution, which is also linear in size.  



Our tool  $\projname$ implements an \emph{exploration-optimal} DPOR algorithm  with linear memory requirements. $\projname$ supports the scoped C/C++ model which includes all axioms of SC as well as relaxed accesses. $\projname$'s explorations of different executions do not share  any states, and it is highly parallelizable. 
On identifying an assertion violation, $\projname$ reports the violation along with the violating execution and 
terminates. On identifying a race or barrier divergence, $\projname$ allows the options of either stopping or continuing until all races/divergences are exposed. In addition, $\projname$ also has an option to fix races; using this option, the user can run $\projname$ iteratively identifying and fixing races until the program is declared free of races. 
We have experimented $\projname$ on several benchmarks to demonstrate its effectiveness. The benchmarks range from small litmus tests to real applications, used in GPU testing \cite{testingGpu,gpuharbor}, bounded model checking \cite{dat3m}, and verification under sequential consistency \cite{Kamath:2020,iguard}. $\projname$ could explore the executions of these benchmarks in a scalable manner and identify the errors. We compare $\projname$ to $\dartagnan$, a bounded model checker for GPU weak memory concurrency \cite{dat3m}. $\projname$ could identify races which are missed by $\dartagnan$ in its benchmarks, and also outperforms $\dartagnan$ significantly 
in terms of memory and time requirements in identifying concurrency errors. 

\paragraph*{Contributions \& Outline}
To summarize our contributions : 
 (1) \Cref{sec:overview} provides an overview of the scoped C/C++ programming model for GPU concurrency, the concurrency errors, and the $\projname$ workflow.
(2)  \Cref{sec:semantics} defines the formal semantic model of scoped C/C++ followed by $\projname$.
    (3) \Cref{sec:dpor} proposes our DPOR algorithm. 
    (4) \Cref{sec:evaluation} discusses the experimental evaluation. 
    (5) We discuss related work in \Cref{sec:related}. 
We provide all proofs in the supplementary material and the $\projname$ model checker is available in \cite{coral-}.



==> introduction-311.tex <==
\section{Introduction}
\label{sec:introduction}
In recent years GPUs have emerged as mainstream processing units, more than just accelerators \cite{8916327_survey_ml,pandey2022transformational_drugdiscovery,ozerk2022efficient_encrypt,francis2014autonomous}. Consequently, beyond parallel programming, \onote{GPUs are becoming} an attractive target for shared memory concurrency for further performance gains. To this end, GPU programming languages such as CUDA and OpenCL, \cite{NVIDIA_CUDA_v12.6,opencl} as well as libraries, \cite{cutlass,cccl} have adopted C/C++ shared memory concurrency primitives.  


Writing correct and highly efficient shared-memory concurrent programs is already a challenging problem, even for CPUs. In addition to the existing challenges, GPU concurrency poses new challenges due to different threading paradigms and scoped memory accesses. Unlike CPU threads, the threads in a GPU are organized hierarchically and synchronize via barriers during execution. Moreover, shared-memory accesses are scoped, resulting in more fine-grained rules for synchronization, based on the proximity of their threads. 
Although these primitives and rules play a key role in achieving better performance, they are also complex and prone to errors. 
 GPU concurrency may result in various types of concurrency bugs -- assertion violations, data races, heterogeneous races, and barrier divergence. While assertion violation and data race errors are well-known in CPU concurrency, they manifest in more complicated ways in the context of GPU programs. The other two types of errors are GPU specific -- heterogeneous races and barrier divergence \sout{errors are exhibited in GPU concurrency, unlike CPUs}. To catch these errors, it is imperative to explore all possible executions of a program. 
 
The set of possible executions of a GPU concurrent program is determined by its underlying consistency model. \scomment{GPU concurrency primitives follow} weak consistency, \scomment{and as a result} a program may exhibit extra behaviors in addition to the interleaving executions -- formally known as sequential consistency \cite{lamport-sc}. 

\scomment{The weak mmeory concurrency models in GPUs differ from the ones in the CPUs. The shared memory accesses in GPUs are scoped and the scopes determine the underlying synchronization rules and consistency model. As a result, }
\sout{Compared to CPUs, GPU concurrency follows weaker consistency models due to the scoped accesses and their weaker synchronization rules.} 
%As a result, they  allow many more  executions. 
The state-of-the-art analysis and verification approaches do not suffice in identifying these errors under GPU weak memory concurrency. As a result, automated reasoning of GPU concurrency, particularly under weak consistency models, even though a timely and important problem,  has remained largely unexplored. 

Stateless model checking(SMC) is a prominent automated verification technique \cite{DBLP:conf/popl/ClarkeES83} that explores the state space of a program in a systematic manner covering all possible executions of the program. However, the number of executions can grow exponentially larger in the number of concurrent programs which poses a key challenge to a model checker. 
To address this challenge, partial order reduction (POR)  \cite{DBLP:journals/sttt/ClarkeGMP99,DBLP:books/sp/Godefroid96,DBLP:conf/cav/Peled93} and subsequently dynamic partial order reduction (DPOR) techniques have been proposed \cite{DBLP:conf/popl/FlanaganG05} to 
explore the executions efficiently without compromising on system coverage. 
\onote{GenMC-Trust \cite{DBLP:journals/pacmpl/Kokologiannakis22} and POP \cite{abdulla2024parsimonious} propose polynomial-space DPOR algorithms.
While these techniques are widely applied for programs written for CPUs including the ones written for weak memory concurrency models, \cite{DBLP:journals/pacmpl/Kokologiannakis18,10.1145/2806886,10.1145/3276505,DBLP:journals/jacm/AbdullaAJS17,DBLP:conf/pldi/Kokologiannakis19,DBLP:journals/pacmpl/Kokologiannakis22}. to our knowledge, this has not been explored for GPU weak memory concurrency. 
GenMC-Trust \cite{DBLP:journals/pacmpl/Kokologiannakis22} and POP \cite{abdulla2024parsimonious} does not support GPU-specific primitives.
}
While these techniques are widely applied for programs written for CPUs including the ones written for weak memory concurrency models, \cite{DBLP:journals/pacmpl/Kokologiannakis18,10.1145/2806886,10.1145/3276505,DBLP:journals/jacm/AbdullaAJS17,DBLP:conf/pldi/Kokologiannakis19,DBLP:journals/pacmpl/Kokologiannakis22}, to our knowledge, this has not been explored for GPU weak memory concurrency. 

\scomment{this paragraph should be moved before SMC}
\noindent{\bf Contributions} To address this gap, in this paper, we develop $\projname$ model checker for a scoped-C/C++ programming languages \cite{Lustig:2019} for GPUs. Scoped-C/C++ has all the shared memory access primitives provided by PTX and Vulkan, and in addition, provide SC memory accesses. \cite{Lustig:2019} formalized the scoped C/C++ concurrency in scoped-RC11 memory model, similar to as C/C++ concurrency is formalized in RC11 \cite{Lahav:2017}. Consequently, $\projname$ is developed for the scoped-RC11 model. 
Besides, the consistency properties defined by scoped-RC11, 
scoped C/C++ programming language follows catch fire semantics similar to traditional C/C++, that is, a program having a scoped-RC11 consistent execution with a data race has undefined behavior. In addition, scoped C/C++ defines \emph{heterogeneous race} for based on the scopes of the accesses and a program having a scoped-RC11 consistent execution with heterogeneous race also has undefined behavior. 

$\projname$ extends the GenMC-TruSt  \cite{DBLP:journals/pacmpl/Kokologiannakis22} approach to handle the GPU-specific features that the original GenMC lacks. 
In particular, these are handling scoped accesses and repairing heterogeneous races.
  $\projname$ implements an \emph{exploration-optimal}, sound and complete DPOR algorithm with linear memory requirements and is parallelizable. 


\kcomment{the  
 scoped RC11 memory model \cite{Lustig:2019}. Soham : can we justify this choice of scoped RC11 upfront?} 
$\projname$ not only reasons about correctness and detects all the errors discussed above but also automatically repair certain errors. More specifically, $\projname$ can fix heterogenous races resulting from mismatches of scopes in GPU programs, thereby progressively transforming a heterogeneous-racy program to generate a heterogeneous-race-free version. 
We empirically evaluate $\projname$ on several benchmarks to demonstrate its effectiveness. The benchmarks range from small litmus tests to real applications, used in GPU testing \cite{Sorensen:2021,gpuharbor}, bounded model checking \cite{dat3m}, and verification under sequential consistency \cite{Kamath:2020,iguard}. 
$\projname$ explores the executions of these benchmarks in a scalable manner and identifies the errors. 
We compare $\projname$ with $\dartagnan$ \kcomment{\cite{hernan24}}, a bounded model checker for GPU weak memory concurrency \cite{dat3m}. $\projname$ identifies races which are missed by $\dartagnan$ in its benchmarks and also outperforms $\dartagnan$ significantly 
in terms of memory and time requirements in identifying concurrency errors. 

% \paragraph{Outline}
% To summarize our contributions : 
%  (1) \Cref{sec:overview} provides an overview of the scoped C/C++ programming model for GPU concurrency, the concurrency errors, and the $\projname$ workflow.
% (2)  \Cref{sec:semantics} discusses the formal semantic model of scoped C/C++ followed by $\projname$. 
%     (3) \Cref{sec:dpor} proposes our DPOR algorithm. 
%     (4) \Cref{sec:evaluation} discusses the experimental evaluation. 
%     (5) We discuss related work in \Cref{sec:related} and conclude in \Cref{sec:conclusion}. 
% We provide all proofs in the supplementary material.
% % and the $\projname$ model checker is available in \cite{coral-}.

%\noindent \textit{Outline}
%(1) \Cref{sec:overview} provides an overview of the scoped C/C++ programming model for GPU concurrency, the concurrency errors, and the $\projname$ workflow.
%(2) In \Cref{sec:semantics} we discuss the formal semantic model of scoped C/C++ followed by $\projname$. 
%    (3) \Cref{sec:dpor} proposes our DPOR algorithm. 
%    (4) In \Cref{sec:evaluation} we present the experimental evaluation. 
%    (5) We discuss related work in \Cref{sec:related} and conclude in \Cref{sec:conclusion}. 
%We provide all proofs in the supplementary material.


==> prelims.tex <==
\section{Preliminaries}
In this section, we first discuss the preliminary notations and the formal definition of the problem of verifying concurrent scoped RC11 programs. 

\Andreas{The color coding is different here from the text. Are we using the same macros?}

\Andreas{Can we replace the included pdfs with tex code for editing?}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{GPU-relations.pdf}
    \caption{Relations in Scoped RC11}
    \label{GPU-relations}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=6cm]{GPU-axioms.pdf}
    \caption{Scoped RC11 Axioms}
    \label{GPU-axioms}
\end{figure}


\noindent{\bf{Concurrent Programs}}. 
A concurrent program $\prog$ consists  of a finite set of \emph{threads} that share a finite set $\varset$  of shared variables 
ranging over a domain $\valset$ of {\em values}. 
  A thread  has a finite set
of local registers that store values from $\valset$.
Each thread is an ordered sequence of labeled instructions built in a standard way from expressions and atomic commands, using standard control
flow constructs (sequential composition, selection, and bounded loop constructs). 
Throughout the paper, we use $\xvar, \yvar, z$ etc for shared variables,
$\areg, \breg, \creg, \dreg, 
r$ for registers. 
 
 The instructions in a thread are write, read, atomic read-modify-write (RMW), assign, fence and barrier  
  instructions, apart from standard conditional flow constructs. 
  Write instructions  write to the shared variable $x$ the value of expression $e$ over local registers while read instructions read from the shared variable $x$
  into a local register $r$. Atomic RMW operations include compare-and-swap (CAS) and fetch-and-add (FADD): in both of these, a read followed by a write to a shared variable is done atomically. Fences and barriers are used for synchronization between threads. A fence is used in one-to-one thread synchronization whereas a barrier ensures that the execution of a program continues only when all threads reach the barrier.    
%  certain point (a ``barrier''). 
We model barriers as acquire-release RMWs on a special auxiliary variable.  

\scomment{All barriers on one variable/different variables?}
\ocomment{Different variables. One variable per workgroup.}


\begin{figure*}
    \includegraphics[width=19cm]{GPU-figs1.pdf}
        \caption{Illustration of scopes, race detection as well as assertion checking}
\label{gpu-egs}
\end{figure*}

\begin{figure}
    \includegraphics[width=9cm]{GPU-figs2.pdf}
        \caption{Scopes, race detection as well as assertion checking}
\label{gpu-egs2}
\end{figure}

  
\noindent{\bf {Events, Execution Graphs and Consistency}}. 
An event corresponds to the effect of executing an instruction in $\prog$. An event 
in a concurrent program $\prog$ is a tuple   $e=(id,\thread,op)$ where 
$id \in \nat$ is the unique identifier of the event, $\thread$ is the thread that performs $e$ 
and $op$ is the operation corresponding to $e$. Often when the $id$ is clear, we drop it. We denote respectively by $e.id, e.\thread$ and $e.op$, the 
$id$ of the event, the thread performing the event and the operation. 
Operations are $\wt(x,v), \rd(x,v)$ (write value $v$ to memory location or variable $x$, or  read $v$ from variable $x$), 
$\rmw(x,v_1,v_2)$ (read modify write by reading $v_1$ from $x$ and writing $v_2$
to $x$). The fetch and add $fadd(x, v, v+1)$ where value $v$ is read from $x$, and the value of $x$ is incremented 
by 1, as well as $cas(x, r_1, r_2)$ where the value of register $r_1$ is read from $x$ and updated with the value of $r_2$ 
are instances of $\rmw(x,v_1,v_2)$. Finally,  we also have the operations of $\fence$ and $\barr$ (fences and barriers).  
Let $\eventset$ denote the set of all events from $\prog$. For $x \in \varset$, let $\eventset^{\wt,x}$ 
denote all the write events on $x$. 


An execution of $\prog$ is a sequence of events. \emph{Execution graphs} or \emph{traces}
are a succinct representation for sets of executions of $\prog$. 
An execution graph  ({\it $\exegraph$} for short)      
$\egraph$ is a tuple $\egraphtuple$. 
$\tpo$ (program order) totally orders events of each thread : 
$e ~\tpo~ e'$ if $e, e'$ are events in the same thread  and   $e.id < e'.id$. 
 For a variable $x$ and events $e, e'$, we have $ e~\rf~e'$ ($e'$ reads from $e$) if 
$e$ is a write event on $x$ and $e'$ is a read event  on $x$. 
 $\co_x$ (modification-order on $x$) is  a total order on the writes per variable $x$, 
and  $\co$ is the union of $\co_x$ for all variables $x$. 
 $\gorder$ is a total order on the events which defines the order in which they are added to  $\egraph$.
 An $\exegraph$ $\mathcal{G}$ is $\valid$ for scoped RC11 (denoted $\valid(\mathcal{G})$) iff it satisfies all axioms given in Figure \ref{GPU-axioms}. 
 
 

\begin{figure*}
    \includegraphics[width=19cm]{GPU-atomicity-fence-nothin.pdf}
        \caption{Illustration of consistency conditions}
\label{GPU-cons}
\end{figure*}
 
 For example, the execution graphs in Figure \ref{GPU-cons}(a)-(d) illustrate 
 violations to coherence, atomicity, SC and the no-thin-air axioms. 
 
  

\subsection{Consistency Model}







\subsection{Examples : Assertion Violation}
In this section, we illustrate examples for assertion violation. These examples also illustrate the various relations used in the scoped RC11 formalization.
 Consider the 5 versions of the standard litmus test \emph{Message Passing} in Figure \ref{gpu-egs}, and the assertion \textbf{forall} $\varphi : r_2 ==1$. 
The assertion violation question is to check if there is an execution which violates $\varphi$. 
  It can be seen that in all these variants, the assertion is violated 
    only when there is no release-acquire synchronization between the threads. 




In Figure \ref{gpu-egs}(a), both threads from the same workgroup. 
The second instruction in the first thread is a release store which synchronizes with ($\sw$) the first acquire read in the second thread. The synchronization
is possible since their scopes are inclusive ($\incl$) : both instructions have a workgroup scope and  the threads  are from the same workgroup. 
 The acquire read in the second thread can read from ($\rf$) the release write of the first thread as a result of the synchronization; this also relates them  
using the happens-before relation, $\hab$. Due to the  synchronization, the value of the local register $r_1$ is 1, and the second acquire read   in the second thread 
cannot read the initial value 0 of $x$ in any execution.   The \textcolor{green}{0//} in green denotes this, and the assertion is not violated in any execution. 


\Andreas{It is ok to use color to aid the reader, but do not rely solely on color. Like above, using the same syntax 0// but different colors (green/red) to denote different things is not good practice.}

In Figure \ref{gpu-egs}(b), the first instruction in the second thread is a relaxed read. 
By definition of $\sw$, the release write on $y$ in the first thread does not synchronize with  a relaxed  read, even though both have 
inclusive scopes and both threads are in the same workgroup.  This also means they are not related by $\hab$. 
 In  Figure \ref{gpu-egs}(c), the second instruction in the first thread and the first instruction in the second thread 
do not synchronize (not related by $\sw$ and $\hab$) since the threads are in different workgroups (hence their scopes are not inclusive).
As a result, the second thread can read the initial value 0 of $y$, and $r_2$ can attain the value 0. 
The  \textcolor{red}{0//} in red denotes this, and we have found an  assertion violation. 

For Figures \ref{gpu-egs}(d), (e), whether the assertion holds or not depends on whether the device scopes $dev_1, dev_2$ are the same, in other words, whether 
the workgroups $wg_1, wg_2$ are in the same device scope. 
If both workgroups are in the same device scope, 
then the release write in the first thread of Figures \ref{gpu-egs}(d),(e) synchronizes (hence related by $\sw, \hab$) with the 
acquire read in the second thread and the assertion is not violated. In both examples,  the scopes of the release write of thread 1 (the second instruction)
as well as the acquire read   of the second thread  (the first instruction) have inclusive scopes (one is $wg$, and the other is $dev$) 
as long as $wg_1,wg_2$ are in the same device scope. Thus, for these examples, we do not comment about 0// in either color. 




\subsection{Examples : Race Detection}
In this section, we give examples of data races. Two memory operations 
are said to conflict when at least one of them is a write, and 
two conflicting memory operations are said to be in a data-race if they are not related in causality order and they are not morally strong. 
Consider the examples in Figure \ref{gpu-egs}. There is no data race in programs Figure \ref{gpu-egs}(a), (b) since the 
conflicting operations are morally strong. Consider Figure \ref{gpu-egs}(c). If the workgroups $wg_1, wg_2$ are different, then 
the conflicting memory operations on $x,y$ in the two threads are not morally strong since their scopes are not inclusive. 
They are also not related by $\hab$, hence not causally related. 
Then there are 2 data races in Figure \ref{gpu-egs}(c) : one between lines 1, 3  and the other between lines 2,1 of the two threads. 
In Figure \ref{gpu-egs}(d),(e) if the two workgroups are not in the same device scope, 
the conflicting memory operations on $x,y$  are not morally strong and not causally related and we get the same two races as in Figure \ref{gpu-egs}(c).

Likewise, for the program in Figure \ref{gpu-egs2}, there is a data race between lines 1,1 of threads 1 and 2. These are non atomic accesses, so 
they are not morally strong, and they are also not related by causality order. The other races are between lines 1 of thread 1 and lines 1,2 of threads 3,4
and likewise lines 1 of thread 2 and lines 1,2 of threads 3,4. 



\subsection{Examples : Consistency Checking}
In this section, we illustrate violation of consistency $(\neg \valid(\mathcal{G}))$ by an execution graph $\mathcal{G}$
on some examples. 



In Figure \ref{GPU-cons}(a), reading the initial value 0 from $x$ by $r_2$ would violate the \emph{coherence} axiom : note that this induces a $\hab;\rb$ cycle from the first instruction of thread 1 to itself. Likewise, assume the $fadd$ operations are not executed atomically in Figure \ref{GPU-cons}(b). One possibility  (as depicted by the execution graph in Figure \ref{GPU-cons}(b)) is when 
the first thread reads value 0 from $x$ and does not increment $x$ immediately. If the control goes to the second thread, then the $fadd$ 
reads 0 from $x$ and writes 1 to $x$. This results in a $\rd$ from thread 1 to 2. 
When control comes back to thread 1, it writes 1 to $x$. This results in an $\co$ from thread 2 to thread 1, obtaining a $\rb;\co$ cycle. A similar 
cycle is obtained if $fadd$ is not executed atomically by thread 2. Note that if both threads execute $fadd$ atomically, 
then $x$ will be 2 at the end.  Figure \ref{GPU-cons}(c) shows violation of the SC axiom if both $r1$ and $r2$ read the initial value 0. In such a case,   
there is a $\tpo;\rb;\tpo;\rb;\tpo$ path from the $\fence.sc$ of thread 1  to itself, constituting a SC violation. Figure \ref{GPU-cons}(d)
 shows violation of the  no-thin-air if $r1$ reads 2 from $y$ and $r2$ reads 1 from $x$. This constitutes a $\tpo$-$\rf$ cycle as seen in 
 Figure \ref{GPU-cons}(d). 














==> seg-dpor-example.tex <==
{
\[
\mytag{SEG}
\label{prg:dpor}
\inarrC{
X=Y=0;
\\[1.2ex]
\inparII{
\T_1\tup{\wg_1, \_}
\\[1.2ex]
X^\wg_\MOrel = 1;
\\[1.1ex]
Y^\wg_\MOrel = 1;
}{
~~\T_2\tup{\wg_1, \_}
\\[1.2ex]
~~a=Y^\wg_\MOna;
\\[1.1ex]
~~b=X^\wg_\MOacq;
}
}
\]
}



==> workflow.tex <==
% \begin{figure}
% \center
% \begin{tikzpicture}
% \node (p) at (0.5,0) {$\mbbp$};
% \node (pf) at (3,-1.5) {$\mbbp_{\mathsf{final}}$};
% \node[draw=black] (mc) at (3,0) {\begin{tabular}{c} Model \\ checking \end{tabular}};
% \node[draw=black] (rp) at (6.5,0) {\begin{tabular}{c} Program \\ repair \end{tabular}};
% %\draw [draw=black] (0,0) rectangle node[]{\begin{tabular}{c} Model \\ checking \end{tabular}} (2.5,1);
% %\draw [draw=black] (4,0) rectangle node[]{Repair} (6,1);


% \draw[->] ([yshift=3mm]mc.east) to node[above]{error} ([yshift=3mm]rp.west);
% \draw[->]  ([yshift=-3mm]rp.west) to node[below]{$\mbbp'$} ([yshift=-3mm]mc.east);
% \draw[->] (mc) to node[left]{no error} (pf);
% \draw[->] (p) to  (mc);
% % \filldraw [fill=Peach, draw=black] (11.1,5) rectangle (0.3,0.3) {fix};
% % \filldraw [fill=RedOrange, draw=black] (11.1,4.5) rectangle (0.3,0.3) {program};
% \end{tikzpicture}
% \caption{Workflow}
% \label{fig:workflow}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=6cm, height=3.5cm]{workflow.eps}
% \caption{Overview of $\projname$}
% \label{fig:workflow}
% \end{figure}


\setlength{\intextsep}{0.5pt}
\setlength{\columnsep}{0.5pt}
\begin{wrapfigure}[9]{r}{0.43\textwidth}
\includegraphics[width=5.6cm, height=3cm]{workflow.eps}
\caption{Overview of $\projname$}
\label{fig:workflow}
\end{wrapfigure}
